You can monitor your hydration level using your smartphone camera

This work proposes for the first time to utilize the regular smartphone -- a popular assistive gadget -- to design a novel, non-invasive method for self-monitoring of one's hydration level on a scale of 1 to 4. The proposed method involves recording a small video of a fingertip using the smartphone camera. Subsequently, a photoplethysmography (PPG) signal is extracted from the video data, capturing the fluctuations in peripheral blood volume as a reflection of a person's hydration level changes over time. To train and evaluate the artificial intelligence models, a custom multi-session labeled dataset was constructed by collecting video-PPG data from 25 fasting subjects during the month of Ramadan in 2023. With this, we solve two distinct problems: 1) binary classification (whether a person is hydrated or not), 2) four-class classification (whether a person is fully hydrated, mildly dehydrated, moderately dehydrated, or extremely dehydrated). For both classification problems, we feed the pre-processed and augmented PPG data to a number of machine learning, deep learning and transformer models which models provide a very high accuracy, i.e., in the range of 95% to 99%. We also propose an alternate method where we feed high-dimensional PPG time-series data to a DL model for feature extraction, followed by t-SNE method for feature selection and dimensionality reduction, followed by a number of ML classifiers that do dehydration level classification. Finally, we interpret the decisions by the developed deep learning model under the SHAP-based explainable artificial intelligence framework. The proposed method allows rapid, do-it-yourself, at-home testing of one's hydration level, is cost-effective and thus inline with the sustainable development goals 3 & 10 of the United Nations, and a step-forward to patient-centric healthcare systems, smart homes, and smart cities of future.

==> sec2.tex <==
\section{Proposed Method for Non-Invasive Dehydration Monitoring}
\label{sec:sys-model}

Our innovative approach utilizes a smartphone's camera to assess an individual's hydration status non-invasively. The process begins with the subject recording a video of their index finger placed on the phone's rear camera, capturing the PPG signal. This raw data goes through several stages of transformation:\\
\textbf{1. Data Acquisition}: Capture of the PPG signal via a smartphone's camera with a video recording of the index finger.
\\\textbf{2. Frames Extraction}: Sequential images are extracted from the video.
\\\textbf{3. Pixel Averaging}: Key pixel values are averaged from the frames to create a time-series data stream.
\\\textbf{4. Time-Series Extraction}: This data is then used to generate a time-series graph that represents the PPG signal.
\\\textbf{5. Pre-processing}: The PPG signal is filtered using a fourth-order Butterworth low-pass filter for noise reduction and then segmented into data samples suitable for analysis.
\\\textbf{6. Classification}: Finally, the pre-processed data is input into advanced neural network models such as LSTM-FCN, BiLSTM, traditional ML classifiers, and Transformers to accurately classify and determine the subject's hydration status.






==> sec3.tex <==
\section{The HCDDM-RF-5 dataset}
\label{sec:method}

This section provides sufficient details about the hardware and software setup used to construct the custom HCDDM-RF-5 dataset\footnote{The acronym HCDDM-RF-5 stands for {\bf H}and and {\bf C}hest {\bf D}ata for {\bf D}ehydration {\bf M}onitoring via {\bf R}adio {\bf F}requency data collected from {\bf 5} subjects.}, our thoughtful data collection methodology (that helped us capture dehydration related data in a very controlled manner), as well as the intricate details of the two experiments performed in order to collect data for the two proposed (CBDM and HBDM) methods. 

%But before this, a quick discussion of the classification problem (hydrated vs. dehydrated) is in order. 

%\subsection{The classification problem}
%The hydrated subject detection problem is reformulated in this work as a classification problem using the categories of hydrated subject and dehydrated subject. The following are some important details for each class.

%Dehydrated class: Ramadan is a holy month in which devout Muslims observe a strict fast from sunrise to sunset. Muslims who are fasting refrain from eating or drinking during this period. We took advantage of this unique opportunity to enlist pious Muslims who were observing a month-long fast. Prior to five minutes before sundown, when subjects were deemed to be dehydrated, we collected 30-second data.

%Hydrated class: After 30 minutes of sunset, when the subject had finished drinking water and eating after breaking the fast (moving from severely dehydrated to hydrated), we took 30-second data and judged the person to be hydrated.

% Tachypnea: Tachypnea occurs when an individual breathes faster than normal. It may be caused by anxiety, shock, exercise, and symptoms of lung disease.

% Bradypnea: Slower breathing as compared to normal breathing is known as Bradypnea. The onset of Bradypnea typically indicates that the body is not getting enough Oxygen. It could also poin to other problems such as Carbon monoxide poisoning, head injury, metabolic disorder, and sleep apnea.

\subsection{USRP SDRs based OFDM transceiver}

%MATLAB's "Communications Toolbox Support Package for USRP Radio" add-on lets the USRP SDR B210 share real-time info with the host PC. In addition, the entire flowgraphs for the transmitter and receiver were designed in Simulink using various building elements (modulators, demodulators, etc.) from the communication system toolbox. 

%We were able to identify and categorise hydrated and dehydrated people on this platform by monitoring minute changes in the wireless channel and collecting detailed CSI. The USRP transmitter consistently broadcasts an RF signal at a fixed frequency, which is then received by a USRP receiver and described in CSI format.
%In MATLAB Simulink, both the transmitter and the receiver are created. Additionally, the USRP SDR is interfaced to the host PC using MATLAB's communication system toolbox. 
% Wireless channel is used to collect information about . The  synthesized generic RF functionality of SDR technology
% recieved signal is described in the form of CSI which captures the minute breathing movements during fasting and after fasting. Later, information retrieved from CSI can be used to detect different breathing patterns which capture human body movements between the two unidirectional (transmit and receive) antennas.

OFDM Transmitter: 
For each OFDM frame, the random bits generator block creates pseudo-random data bits with a chunk size of 128 bits. The QPSK modulator block maps these bits to (frequency domain) symbols which are then transformed into a time-domain signal by means of an inverse fast Fourier transform (IFFT) of size $N=64$ points. Further, a cyclic prefix (CP) of size 16 samples is appended to each OFDM frame, making each OFDM frame 80 samples long. Gain of the transmit horn antenna is set to 40 dB. Fig. 2(a) shows the Simulink flowgraph of USRP SDR based OFDM transmitter.

OFDM Receiver: 
After removing the CP from each OFDM frame, fast Fourier transform (FFT) is then used to transform the received time-domain OFDM samples into the equivalent frequency-domain OFDM symbol. Then, keeping in mind that the transmitted QPSK symbols on each sub-carrier are known to the OFDM receiver, the channel coefficient $h_i$ for $i$-th sub-carrier could simply be computed as: $h_i=\frac{y_i}{x_i}$, where $x_i$,$y_i$ are the transmitted and received QPSK symbol on $i$-th sub-carrier, respectively. This way, the raw CFR data $\mathbf{h}=[h_1,\cdots,h_N]^T$ is collected by the OFDM transmitter, which is to be utilized later by the ML algorithms in order to classify the status of each subject as either hydrated or dehydrated.
Fig. 2(b) shows the Simulink flowgraph of USRP SDR based OFDM transmitter.

% Then, the amplitude response of the frequency domain signal is  extracted to classify the dehydrated subject.
% The SDRu source block is employed to configure the hardware parameters of the receive USRP SDR (see Table \ref{table:1}), and to receive baseband samples from USRP B210. The gain of receive horn antenna is set to 40 dB. The first step of the receive flowgraph is to identify the start of the OFDM frame in order to remove the 16 samples corresponding to CP. This is followed by an FFT block that returns the noisy OFDM symbol. Next, complex-valued CFR is extracted, which is one of the many manifestations of the CFR. The variation in CFR arises due to channel effects and is investigated to sense breathing abnormalities. Fig. \ref{fig:flowg} (b) shows the transmitter flowgraph used to program the receive USRP SDR.

{Table \ref{table:1} provides a quick summary of setting of various relevant parameters of transmit and receive USRP SDRs.}

\begin{figure*}
\hfill
\subfigure[The transmitter flowgraph]{\includegraphics[scale=0.42]{Figures/MAtlab_simulink_Tx.png}}
\hfill
\subfigure[The receiver flowgraph]{\includegraphics[scale=0.42]{Figures/MATLAB_simulin_diagram_Rx}}
\hfill
\caption{The Simulink flowcharts of the USRP-SDR based OFDM transmitter and receiver. }
\label{fig:flowg}
\end{figure*}

%needs to populate it.
\begin{table}[h!]
\centering
\begin{tabular}{|c| c|} 
 \hline
 
 {Parameter} & {Type/Value}
	
\\
\hline


Bits per OFDM frame &	$128$ \\
Bits per symbol &	$2$ \\
Coding scheme &	Gray coding
 \\
Modulation scheme &	QPSK \\
No. of OFDM subcarriers (N) &	$64$\\
Data subcarriers &	$52$\\
Pilot subcarriers &	$12$\\
Size of FFT/IFFT &	$64$ points\\
Size of cyclic prefix	& $16$\\
Sampling rate&	$20,000$ samples/sec\\
Antenna type&	directional horn \\
USRP B210 frequency range&	$70$ MHz - $6$ GHz\\
Centre frequency&	$5.23$ GHz\\
Clock source \& PPS source &	Internal\\
Internal clock rate &	$200$ MHz\\
Interpolation factor (at Tx) &	$250$\\
Decimation factor (at Rx) &	$250$\\
Transmitter gain (at Tx and Rx) &	$40$ dB\\

 \hline
\end{tabular}
\caption{Some parameters for the USRP-SDR-based OFDM transceiver used for non-contact monitoring of dehydration.}
\label{table:1}
\end{table}



\subsection{Data Acquisition for the HCDDM-RF-5 dataset}
%Extensive studies are run to assess the platform's performance in identifying and categorising the dehydrated subject after the transmitter and receiver have been designed.
The custom HCDDM-RF-5 dataset was constructed by collecting data from five volunteers during the month of Ramadan (between March 23rd, 2023 and April 21st, 2023). Ramadan is an  holy month during which devout Muslims observe a strict fast from sunrise till sunset. That is, while they are fasting, Muslims refrain from eating and drinking from sunrise till sunset. We took advantage of this unique opportunity in order to collect dehydration related data from five devout Muslims who had been fasting during this month. Among five subjects, two were males (aged 28, 62 years), and three were females (aged 21, 26, 61 years). For each fasting subject, we collected data twice, once for each class label (hydrated and dehydrated) in order to construct a balanced dataset. Specifically, first episode of data collection took place about 30 minutes before the sunset when the subject was deemed to be maximally dehydrated (thus, this data belongs to the first/dehydrated class). Subsequently, the second episode of the data collection took place an hour after the sunset, after the subject had finished eating and drinking after breaking the fast (thus, this data belongs to the second/hydrated class). For each subject, we conducted two kinds of experiments where we exposed the subject's chest and hand to the RF signals, respectively. Some more pertinent details about data collection for our proposed CBDM and HBDM methods are given below. 

% During the first set of experiments, we collected data from the chest movement, whereby the transmitter SDR impinges the signal onto the chest of the subject, while the receiver SDR collects the signal reflected off the body (see Fig. \ref{fig:method1}). The second set of experiments represents the proposed method where the subject places his/her hand on a table such that the transmitted signal passed through the hand, and the weak signal that penetrates through the hand is collected at the receiving end (see Fig. \ref{fig:methodour}). 

% It is worth mentioning that the first set of experiments was done in order to utilize the work \cite{benchmarkworkQammer} as a benchmark to assess the performance of our proposed method against it. 

{\it Data collection for the proposed CBDM method:} 
During data acquisition for the proposed CBDM method, each participant sat on a chair that was about 80 cm away from the pair of directional horn antennas that pointed towards the chest of the subject (see Fig. 3). As described before, the transmit horn antenna impinged an OFDM signal onto the chest of the subject, while the receive horn antenna gathered the signal reflected off the subject's chest. During each experiment session, the subject sat still in order to avoid motion-induced artefacts in the data being gathered. Each single experiment session lasted for 30 seconds. For each subject, we conducted five experiment sessions before the sunset (to capture the raw CFR data for dehydrated class) and five experiment sessions after the sunset (to capture the raw CFR data for the hydrated class). This way, we were able to collect $30\times5=150$ seconds worth of data for each class (for a given subject), and thus, $150\times2=300$ seconds worth of data per subject. Ultimately, for 5 subjects, this led to a total dataset size of $300\times5=1500$ seconds (or, 25 minutes) of raw CFR data (that corresponds to a total of $5\times5\times2=50$ experiment sessions). 
% The essential figures from the data collection for the experiment based on chest movement are presented in the following table. The experimental setup for the data collection campaign for the benchmark approach is shown in Fig. (a).

\begin{figure}[ht]
\begin{center}
	\includegraphics[width=8cm,height=4cm]{Figures/Chest_movment_based_experiment.drawio (1).png} 
\caption{Experimental setup of the proposed CBDM method.}
\label{fig:method1}
\end{center}
\end{figure}

{\it Data collection for the proposed HBDM method:} 
%Two USRP radios each linked to the host PC are set up on a table with their directional horn antennas (separated by 60 cm) facing in the direction of each other, as shown in Fig. $4$. The individual places a hand on the table between the transmit and receive horn antennas while seated in a chair close to them. As before, the subject's hand is impinged with an OFDM signal by the transmit horn antenna, while the receive horn antenna gathers the faint signal that successfully passes through the subject's hand. 
During data acquisition for the proposed HBDM method, each participant sat on a chair that was about 60 cm away from the pair of directional horn antennas facing each other, and placed his/her hand on the table between the two antennas (see Fig. 4). Again, the transmit horn antenna impinged an OFDM signal onto the hand of the subject, while the receive horn antenna gathered the signal passed through the subject's hand. During each experiment session, the subject sat still in order to avoid motion-induced artefacts in the data being gathered. The rest of the details of data acquisition for the proposed HBDM method are the same as before. That is, for each subject, we conducted five experiment sessions before the sunset (to capture the raw CFR data for dehydrated class) and five experiment sessions after the sunset (to capture the raw CFR data for the hydrated class). This way, for 5 subjects, we acquired a dataset that consisted of $300\times5=1500$ seconds (or, 25 minutes) of raw CFR data (that corresponds to a total of $5\times5\times2=50$ experiment sessions). 

In short, combining the two smaller datasets due to CBDM method and HBDM method together, the custom HCDDM-RF-5 dataset consists of a total of 50 minutes of raw CFR data that corresponds to a total of 100 experiment sessions. 


%As breathing rate affects the blood flow in the whole body e.g. slow breathing triggered the parasympathetic nervous system which results in decreasing heart rate and widening the blood vessel. These small-scale movements are captured by CFR (for all OFDM subcarriers).

\begin{figure}[ht]
\begin{center}
	\includegraphics[width=9cm,height=3cm]{Figures/hand_movment_based_experiment.drawio.png} 
\caption{Experimental setup of the proposed HBDM method. }
\label{fig:methodour}
\end{center}
\end{figure}

% \subsection{Data Acquisition}
% We recruit 5 participants during the month of Ramadan (between March 23rd, 2023
% and April 21rd, 2020 ). The month of Ramadan is a holy month when religious Muslims honor this special month by fasting from sunrise to sunset. During this time, fasting Muslims do not take any foods or drinks. We took advantage of this special occasion and recruited 5 religious Muslims who were fasting for a month. We collected 30-second data just 5 minutes before sunset which time participants were considered as dehydrated.  Additionally, We collected 30-second data after 30 minutes of the sunset, when he/she finished taking water and food by breaking the fasting (transition from very dehydrated to hydrated) and now participants were considered as hydrated. 
% {\it Data acquisition for chest movement-based: } 
% Data is collected in the lab environment. Four healthy volunteers (all males) participated in the data collection campaign. Each subject was requested to perform three different breathing activities (Eupnoea, Tachypnea, and Bradypnea) artificially. In other words, each subject breathed normally for Eupnoea experiment, underwent fast breathing for Tachypnea experiment, and performed slow breathing for Bradypnea experiment. Furthermore, the experiment for each breathing activity for each subject was repeated five times. Each experiment (transmission) lasted for 30 seconds. This led to a total of $4\times 3\times 5=60$ experiments. The data collected after each experiment consisted of the complex-valued CFR (a manifesttaion of the WSCI). Table \ref{table:datasetref} summarizes the key statistics of the data collection done for the chest movement-based experiment. Fig. \ref{fig:real_exp_pics} (a) shows the experimental setup used for data acquisition campaign for the benchmark method.

% {\it Data acquisition for proposed method (hand movement-based): }
% The data acquisition campaign for hand movement-based experiment is completely identical to the data collection campaign for the first experiment. That is, 4 volunteers performed 3 breathing activities while repeating each activity 5 times, thus giving rise to a total of 60 experiments. However, note that the subjects were advised to keep their hand (under test) static on the table between the transmit and receive horn antenna, while performing different breathing activities. This was to make sure that there are no motion-induced artefacts in the data being collected (which would in turn help in capturing the very subtle/minute movement of hand due to respiration). Table \ref{table:datasetref} could again be referred to, to get a quick glimpse at the key statistics of the data collected for the hand-movement based experiment. Fig. \ref{fig:real_exp_pics} (b) shows the experimental setup used for data acquisition campaign for the proposed method.

% \begin{figure*}
% \hfill
% \subfigure[Data collection for benchmark method]{\includegraphics[scale=0.2]{Figures/Sys_RM.jpeg}}
% \hfill
% \subfigure[Data collection for proposed method]{\includegraphics[scale=0.2]{Figures/Sys_PM.jpeg}}
% \hfill
% \caption{Data acquisition campaign: benchmark method (left), and the proposed method (right)}
% \label{fig:real_exp_pics}
% \end{figure*}

%needs to populate it.
% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c|} 
%  \hline
%  Parameter & Value
	
% \\
% \hline
% Number of subjects&	$5$ \\
% Number of classes &	$3$ \\
% Number of times each activity was performed &	$5$ \\
% Duration of each experiment &	$30$ sec \\
% Total number of experiments&	$60$ \\
% Number of USRP radios used &	$2$ \\
% Number of PCs used &	$2$ \\

%  \hline
% \end{tabular}
% \caption{Specifics of the data gathering effort that will be required for the proposed methodology  }
% \label{table:datasetref}
% \end{table}





==> sec4.tex <==
\section{Training and Testing of Machine Learning Classifiers}

For the binary classification problem (hydrated/dehydrated) under consideration, we train and test the following five ML classifiers and their variants: K-nearest neighbours (KNN), support vector machine (SVM), decision tree (DT), ensemble classifier, and neural network. 
Subsequently, we provide detailed performance analysis and comparison of all the ML classifiers implemented. 

\subsection{Data Pre-processing \& Training of Machine Learning Classifiers }  

{\it Data Pre-processing:}
We utilised a low-pass filter and a Savitzky-Golay filter to denoise the CFR extracted from the received OFDM signal, for all the experiment sessions (for both CBDM and HBDM methods). We inspected the whole data manually and removed artifacts where found.

{\it Training \& validation of ML classifiers: }
The Matlab's classification learner app was used to train the following ML classifiers:
K-nearest neighbour (KNN), support vector machine (SVM), decision tree (DT), ensemble classifier, and neural network. All the classifiers were trained on both labelled datasets (corresponding to the CBDM method and the HBDM method). The K-fold cross-validation strategy was used for validation in order to prevent the over-fitting issue. 

%Remember that the dataset is randomly split into smaller portions for training and testing in the cross-validation approach. For instance, if K is 5, 80 percent of the data would be used for training and the remaining 20 percent will be used for testing and validation. 
% The classifier model will train five times if K=5. 


\subsection{Performance metrics}

Each classifier's performance is quantified in terms of accuracy, given as: 
\begin{align}
   & \mathrm{Accuracy}=\frac{\mathrm{Correct \; prediction}}{\mathrm{Total \; observations}}\times 100
\\
&\mathrm{Accuracy}=\frac{T_n+T_p}{T_n+T_p+F_n+F_p} \times 100  
\end{align}
where $T_n$ represents a true negative, $T_p$ represents a true positive, $F_n$ represents a false negative, and $F_p$ represents a false positive. In addition, we also do a performance comparison of the various ML algorithms by means of a confusion matrix.
% and mismatch for breathing
% experiment data are presented in Table 6. The performance analysis of algorithms for
% breathing experiments data are presented in Table 7.
% This section discusses the performance of the proposed SDR-based, ML-empowered non-contact method that captures the subtle but periodic movements of the chest as well as hand for the detection of dehydrated subjects. 

% Additionally, we also construct the confusion matrices in order to investigate the test accuracy of the three ML classifiers. 

\subsection{Performance of proposed CBDM method }
%Recall that the proposed CBDM method classifies dehydrated people based on the radio data collected off the chest.

We begin with performance analysis of the k-NN classifier for three distinct values of k, i.e., k=1,k=10,k=100 (where k is the number of neighbours used to calculate the distance to the new data point). We learn that the fine k-NN (k=1) achieves an accuracy of 79.1$\%$, medium k-NN (k=10) achieves an accuracy of 69.2$\%$, while the coarse K-NN (k=100) achieves a very low accuracy of 55.3$\%$ (see Fig. 5 that displays the detailed confusion matrix).

Next, we focus on Fig. 6 and do performance comparison of the remaining four ML classifiers (and their variants). Beginning with an SVM classifier (with linear, quadratic, and cubic kernels), we note that the linear SVM achieves an overall accuracy of 86.5\%, quadratic SVM achieves an overall accuracy of 89.6\%, while the cubic SVM achieves an overall accuracy of 90.9\%. 
Next, we focus on the decision tree classifier, and note that it has the lowest accuracy of all. That is, the fine tree (despite its many leaves and despite its ability to differentiate between classes precisely) achieved an accuracy of 68.8\% only, while the coarse tree achieved a very low accuracy of 58.0\% only. 
Next in line is the ensemble classifier (a mixture of many classifiers) that is typically implemented with the aim to boost classification accuracy. We observe the following: the ensemble boosted tree has an overall accuracy of 70.3\%, the ensemble bagged tree has an accuracy of 77.9\%, the ensemble subspace KNN has an accuracy of 82.9\%, while the ensemble subspace discriminant has an accuracy of 89.6\%. 
Finally, the neural network (NN) classifier. Each variant of the NN classifier is a fully-connected feedforward network. After each fully connected layer, the Relu activation function is applied, except the last year where softmax activation function is used. We observe that all the different variants of the NN classifier outperform the other ML classifiers. Specifically, the narrow variant of the neural network achieves an accuracy of 93.8\%, the medium neural network achieves an accuracy of 92.5\%, the broad neural network achieves an accuracy of 92.9\%, the bi-layered variant of neural network achieves an accuracy of 93\%, while the tri-layered variant of the neural network achieves an accuracy of 93.1\%. 

Fig. $7$ provides an alternate way of comparing the overall accuracy of all the five ML classifiers and their variants. We note that, for the proposed CBDM method, the neural network classifier (with the narrow neural network) achieves the highest accuracy, which is 93.8\%.

\begin{figure}[t]
\begin{center}
	\includegraphics[scale=0.3]{K_NN_1.pdf} 
\caption{Confusion matrix of k-NN algorithm for the proposed CBDM method.}
\label{fig:methodour}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
	\includegraphics[scale=0.35]{chest_based_confusion_matrix.pdf} 
\caption{Confusion matrix of each of SVM, DT, Ensemble classifiers, and NN for the proposed CBDM method.}
\label{fig:methodour}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
	\includegraphics[scale=0.33]{Chest_Accu.pdf} 
\caption{Performance comparison of all the classifiers for the proposed CBDM method.}
\label{fig:methodour}
\end{center}
\end{figure}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithm &
% 	Actual /Predicted&	Hydrated &	Dehydrated
% \\
% \hline

%  &	Hydrated &	\cellcolor{blue!25}73.7 & 26.3 \\
% k-NN
% (k=1) &		Dehydrated &	15.5 &	\cellcolor{blue!25}84.5  \\

% \hline 

%  &	Hydrated &	\cellcolor{blue!25}60.2 & 39.8 	 \\
% k-NN
% (k=10) &	Dehydrated&	21.9 &	\cellcolor{blue!25}78.1  \\

 
% \hline 

% 	& Hydrated &	\cellcolor{blue!25}21.1 &	78.9 \\
% k-NN
% (k=100) &	Dehydrated &	10.4 &	\cellcolor{blue!25}89.6  \\

 
%  \hline
% \end{tabular}
% \caption{Confusion matrix of k-NN algorithm for the chest movement-based method.} 
% % Total number of observations for each breathing class is 1280. }
% \label{table:knnref}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithm &
% 	Actual /Predicted&	Hydrated &	Dehydrated	
% \\
% \hline
%  &	Hydrated &	\cellcolor{blue!25}87.4 & 12.6 \\
% Linear SVM &		Dehydrated &	14.4 &	\cellcolor{blue!25}85.6  \\
 
% \hline 
%  &	Hydrated &	\cellcolor{blue!25}88.5 &	11.5 \\
% Quadratic SVM&	Dehydrated &	9.3 &	\cellcolor{blue!25}90.7 \\

% \hline 
%  &	Hydrated &	\cellcolor{blue!25}89.4 &	10.6 \\
% Cubic SVM&	Dehydrated &	7.6 &	\cellcolor{blue!25}92.4 \\

% \hline 

%  & Hydrated &	\cellcolor{blue!25}68.0 &	32.0  \\
% DT (Fine Tree) &	Dehydrated &	30.3 &	\cellcolor{blue!25}69.7 \\

%  \hline
% 	& Hydrated &	\cellcolor{blue!25}99.1 &	0.9  \\
% DT (Coarse Tree) &	Dehydrated &	83.2 &	\cellcolor{blue!25}16.3 \\

%  \hline
%%%%%%%%%%%
% Ensemble	& Hydrated &	\cellcolor{blue!25}76.2 &	23.8  \\
%  Boosted Tree &	Dehydrated &	35.6 &	\cellcolor{blue!25}64.4 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}82.1 &	17.9  \\
%  Bagged Tree &	Dehydrated &	26.4 &	\cellcolor{blue!25}73.6 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}77.9 &	22.1  \\
%  Subspace KNN &	Dehydrated &	12 &	\cellcolor{blue!25}88.0 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}88.9 &	11.1  \\
%  Subspace Discriminant &	Dehydrated &	9.7 &	\cellcolor{blue!25}90.3 \\

%  \hline
% %%%%%% NN
% Narrow	& Hydrated &	\cellcolor{blue!25}93.2 &	6.8  \\
%  Neural Network &	Dehydrated &	5.6 &	\cellcolor{blue!25}94.4 \\

%  \hline
%  Medium	& Hydrated &	\cellcolor{blue!25}91.4 &	8.6  \\
%  Neural Network &	Dehydrated &	6.3 &	\cellcolor{blue!25}93.7 \\

%  \hline
%  Wide & Hydrated &	\cellcolor{blue!25}91.6 &	8.4  \\
%  Neural Network &	Dehydrated &	5.8 &	\cellcolor{blue!25}94.2 \\

%  \hline
%  Bilayered	& Hydrated &	\cellcolor{blue!25}93.0 &	7.0  \\
%  Neural Network &	Dehydrated &	7.1 &	\cellcolor{blue!25}92.9 \\

%  \hline
%  Trilayered	& Hydrated &	\cellcolor{blue!25}92.8 &	7.2  \\
%  Neural Network &	Dehydrated &	93.4 &	\cellcolor{blue!25}6.6 \\

%  \hline
 
% \end{tabular}
% \caption{Confusion matrix of SVM, DT, and Ensemble classifiers for the chest movement-based method . }
% % Total number of observations for each breathing class is 1280.}
% \label{table:svmdtref}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c|} 
%  \hline
%  Algorithm &
% 	Accuracy
% \\
% \hline
% Fine k-NN (k=1) & 79.1$\%$ \\
% Medium k-NN (k=10) & 69.2$\%$ \\
% Medium k-NN (k=100) & 55.3$\%$ \\
% \hline 
% Linear SVM & 86.5$\%$ \\
% Quadratic SVM & 89.6$\%$ \\
% Cubic SVM & 90.9$\%$ \\
% \hline 
% DT (Fine Tree) & 68.8$\%$ \\
% DT (Coarse Tree) & 58.0$\%$ \\
%  \hline
% Ensemble Boosted Tree & 70.3$\%$ \\
% Ensemble Bagged Tree & 77.9$\%$ \\
% Ensemble Subspace KNN & 82.9$\%$ \\
% Ensemble Subspace Discriminant & 89.6$\%$ \\
%  \hline
% Narrow Neural Network & 93.8$\%$ \\
% Medium Neural Network Tree & 92.5$\%$ \\
% Wide Neural Network & 92.9$\%$ \\
% Bilayered Neural Network & 93.0$\%$ \\
% Trilayered Neural Network & 93.1$\%$ \\
%  \hline
% \end{tabular}
% \caption{Performance comparison of all the classifiers for the chest movement-based method.}
% \label{table:refmoverall}
% \end{table}
\subsection{Performance of proposed HBDM method}
%Recall that the proposed HBDM method utilizes the radio signals reflected off the hand in order to make its determinations.

%Fig. $8$ gives a comprehensive confusion matrix that distinguishes between the k-NN (fine, medium, coarse), SVM (linear, quadratic, and cubic), DT (fine, and coarse), ensemble classifiers(boosted tree and bagged tree), and neural network (narrow, medium, wide, bilayered, and trilayered) in terms of accuracy. 


% Table  provides the detailed confusion matrix showing the performance breakup of the  k-NN , SVM (linear, quadratic, and cubic), DT (fine, and coarse), ensembled classifiers (boosted tree, bagged tree, subspace KNN, and subspace discriminant), and neural network (narrow, medium, wide, bilayered, and trilayered). We note that both the fine k-NN (k=1) and medium k-NN (k=3) perform poorly as they obtain an overall accuracy of 45.7$\%$ and 45.9\%, respectively. On the other hand, linear SVM and quadratic SVM perform very well with an overall accuracy of 88.1 $\%$ and 85.7$\%$, respectively. The DT algorithm performs the worst with an overall accuracy of 40.8$\%$. 
% Table  provides a compact summary of overall performance of the three classifiers. The SVM classifier (with linear kernal) performs the best with an overall accuracy of $88.1$\%, for the proposed method (which capitalizes on very minute but rhythmic movements of the hand due to respiration for breathing pattern classification).
%Fig. $9$ summarises the classifiers' overall performance in a concise format. For the hand based method, the neural network classifier (with medium layers) achieves the highest accuracy, 88.1. 

We begin performance analysis of our proposed HBDM method from Fig. 8 which provides confusion matrix of each of five ML classifiers (and their variants). 
Beginning with an SVM classifier (with linear, quadratic, and cubic kernels), we note that the linear SVM achieves an overall accuracy of 71.1\%, quadratic SVM achieves an overall accuracy of 89.2\%, while the cubic SVM achieves an overall accuracy of 88.2\%. 
Next, the decision tree classifier. We observe that once again it has the lowest accuracy of all. That is, the fine tree achieved an accuracy of 72.2\% only, while the coarse tree achieved a very low accuracy of 61.4\% only. 
Next, the ensemble classifier. We observe the following: the ensemble boosted tree has an overall accuracy of 74.8\%, while the ensemble bagged tree has an accuracy of 79.7\%. 
Finally, the neural network (NN) classifier. Once again, all the different variants of the NN classifier outperform the other ML classifiers. Specifically, the narrow variant of the neural network achieves an accuracy of 94.7\%, the medium neural network achieves an accuracy of 96.15\%, the broad neural network achieves an accuracy of 95.15\%, the bi-layered variant of neural network achieves an accuracy of 92.35\%, while the tri-layered variant of the neural network achieves an accuracy of 94.2\%. 

Fig. 9 provides an alternate way of comparing the overall accuracy of all the five ML classifiers and their variants. We note that, for the proposed HBDM method, the neural network classifier (with the medium neural network) achieves the highest accuracy, which is 96.15\%.

\subsection{Performance comparison with the state-of-the-art}
Finally, Table II compares the accuracy of the proposed non-contact CBDM and HBDM methods with the state-of-the-art methods which are all contact-based methods for dehydration monitoring. Compared to the state-of-the-art where the maximum reported accuracy is 97.83\%, our proposed non-contact method is slightly inferior (as we report a maximum accuracy of 96.15\%); nevertheless, the advantages of
our non-contact dehydration method speak for themselves. That is, our proposed method is non-invasive and contact-less, has high accuracy, allows continuous and seamless monitoring, is easy to use, and provides rapid results.  


\begin{figure}[t]
\begin{center}
	\includegraphics[scale=0.33]{Figures/hand_based_confu.pdf} 
\caption{Confusion matrix of each of KNN, SVM, DT, Ensemble classifiers, and NN for the proposed HBDM method.}
\label{fig:methodour}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
	\includegraphics[scale=0.33]{Figures/hand_Accu.pdf} 
\caption{Performance comparison of all the ML classifiers for the proposed HBDM method.}
\label{fig:methodour}
\end{center}
\end{figure}




% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithms &
% 	Actual /Predicted&	Hydrated &	Dehydrated
% \\
% \hline
% &	Hydrated &	\cellcolor{blue!25}79.6 & 20.4 \\
% k-NN (k=1)&		Dehydrated&	14.1 &	\cellcolor{blue!25}85.9 \\

% \hline
% &	Hydrated &	\cellcolor{blue!25}69.2  & 30.8 \\
% k-NN (k=10)&		Dehydrated&	26.5&	\cellcolor{blue!25}73.5\\
% \hline
% &	Hydrated &	\cellcolor{blue!25}25.3& 74.8 \\
% k-NN (k=100)&		Dehydrated&	13& 	\cellcolor{blue!25}87.0 \\

% \hline
% &	Hydrated &	\cellcolor{blue!25}46.7 & 53.3 \\
% Linear SVM &		Dehydrated&	4.4&\cellcolor{blue!25}	95.6\\

% \hline 
% &	Hydrated&	\cellcolor{blue!25}85.3&	14.7 \\
% Quad. SVM&	Dehydrated&	7.0&	\cellcolor{blue!25}93.0 \\

% \hline 
% &	Hydrated&	\cellcolor{blue!25}87.1&	12.9 \\
% Cubic SVM&	Dehydrated&	10.6&	\cellcolor{blue!25}89.4 \\

% \hline 
% 	&Hydrated&	\cellcolor{blue!25}&	3.30 \\
% DT &	Dehydrated&	80.40&	\cellcolor{blue!25}13.12\\

%  \hline
%  &Hydrated&	\cellcolor{blue!25}91.32&	3.30 \\
% DT &	Dehydrated&	80.40&	\cellcolor{blue!25}13.12\\

%  \hline
%  Ensemble	& Hydrated &	\cellcolor{blue!25}76.2 &	23.8  \\
%  Boosted Tree &	Dehydrated &	35.6 &	\cellcolor{blue!25}64.4 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}82.1 &	17.9  \\
%  Bagged Tree &	Dehydrated &	26.4 &	\cellcolor{blue!25}73.6 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}77.9 &	22.1  \\
%  Subspace KNN &	Dehydrated &	12 &	\cellcolor{blue!25}88.0 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}88.9 &	11.1  \\
%  Subspace Discriminant &	Dehydrated &	9.7 &	\cellcolor{blue!25}90.3 \\

%  \hline
% %%%%%% NN
% Narrow	& Hydrated &	\cellcolor{blue!25}93.2 &	6.8  \\
%  Neural Network &	Dehydrated &	5.6 &	\cellcolor{blue!25}94.4 \\

%  \hline
%  Medium	& Hydrated &	\cellcolor{blue!25}91.4 &	8.6  \\
%  Neural Network &	Dehydrated &	6.3 &	\cellcolor{blue!25}93.7 \\

%  \hline
%  Wide & Hydrated &	\cellcolor{blue!25}91.6 &	8.4  \\
%  Neural Network &	Dehydrated &	5.8 &	\cellcolor{blue!25}94.2 \\

%  \hline
%  Bilayered	& Hydrated &	\cellcolor{blue!25}93.0 &	7.0  \\
%  Neural Network &	Dehydrated &	7.1 &	\cellcolor{blue!25}92.9 \\

%  \hline
%  Trilayered	& Hydrated &	\cellcolor{blue!25}92.8 &	7.2  \\
%  Neural Network &	Dehydrated &	93.4 &	\cellcolor{blue!25}6.6 \\

%  \hline

 
% \end{tabular}
% \caption{Confusion matrix of the three classifiers for the proposed method (hand movement-based). Total number of observations for each breathing class is 1280.}
% \label{table:confmatprop}
% \end{table}


% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c|} 
%  \hline
%  Algorithm &
% 	Accuracy
% \\
% \hline
% Fine k-NN (k=1) & 82.8$\%$ \\
% Medium k-NN (k=10) & 69.2$\%$ \\
% Medium k-NN (k=100) & 55.3$\%$ \\
% \hline 
% Linear SVM & 86.5$\%$ \\
% Quadratic SVM & 89.6$\%$ \\
% Cubic SVM & 90.9$\%$ \\
% \hline 
% DT (Fine Tree) & 68.8$\%$ \\
% DT (Coarse Tree) & 58.0$\%$ \\
%  \hline
% Ensemble Boosted Tree & 70.3$\%$ \\
% Ensemble Bagged Tree & 77.9$\%$ \\
% Ensemble Subspace KNN & 82.9$\%$ \\
% Ensemble Subspace Discriminant & 89.6$\%$ \\
%  \hline
% Narrow Neural Network & 93.8$\%$ \\
% Medium Neural Network Tree & 92.5$\%$ \\
% Wide Neural Network & 92.9$\%$ \\
% Bilayered Neural Network & 93.0$\%$ \\
% Trilayered Neural Network & 93.1$\%$ \\
%  \hline
% \end{tabular}
% \caption{Performance comparison of all the three classifiers for the proposed method (hand movement-based).}
% \label{table:propmoverall}
% \end{table}




 \begin{table}[h!]
\centering
\begin{tabular}{|c| c|} 
 \hline
 Work &
	Accuracy
\\
\hline
Liaqat et al. \cite{liaqat2022personalized} & 97.83$\%$ \\
\hline
Kulkarni et al. \cite{kulkarni2021non} & 75.96$\%$ \\
\hline
Liaqat et al. \cite{liaqat2020non} & 91.53$\%$ \\
\hline 
Rizwan et al \cite{rizwan2020non} & 85.63$\%$ \\
\hline 
Carrieri et al. \cite{carrieri2020explainable} & 73.91 $\%$ \\
\hline  
Our non-contact CBDM method & 93.8$\%$ \\
\hline 
Our non-contact HBDM method & 96.15$\%$ \\
\hline 

\end{tabular}
\caption{Accuracy comparison of our proposed non-contact CBDM and HBDM methods with the state-of-the-art (contact-based methods). }
\label{table:propmoverall}
\end{table}






% We presented in detail the performance results of all the classifiers for both methods (i.e., exploits the chest movement, and rhythmic hand movements). The results point towards a tradeoff: the hand movement-based method has slightly lower accuracy than the chest movement-based method (95.9\% vs. 88.1\%), but the hand movement-based method will expose the subjects to the least amount of potentially harmful radiation (full chest vs. a hand only). We further notice that the performance of the proposed methods may further be increased by implementing the state-of-the-art deep learning methods which will require a very large dataset in order to train (leading to a very extensive data collection campaign).

% A key benefit of the proposed methods is that they could lead to the development of a smart mobile health (m-health) solution that could be deployed in remote areas far away from mega cities in order to ensure the comprehensive health monitoring of the people in those areas. Additionally, the proposed method could prove to be very useful for rapid and non-contact testing of masses for their respiratory performance during the outbreak of a pandemic like covid19.


